A Pointer Network-based Approach for Joint Extraction and Detection of Multi-Label Multi-Class Intents

In task-oriented dialogue systems, intent detection is crucial for interpreting user queries and providing appropriate responses. Existing research primarily addresses simple queries with a single intent, lacking effective systems for handling complex queries with multiple intents and extracting different intent spans. Additionally, there is a notable absence of multilingual, multi-intent datasets. This study addresses three critical tasks: extracting multiple intent spans from queries, detecting multiple intents, and developing a multi-lingual multi-label intent dataset. We introduce a novel multi-label multi-class intent detection dataset (MLMCID-dataset) curated from existing benchmark datasets. We also propose a pointer network-based architecture (MLMCID) to extract intent spans and detect multiple intents with coarse and fine-grained labels in the form of sextuplets. Comprehensive analysis demonstrates the superiority of our pointer network-based system over baseline approaches in terms of accuracy and F1-score across various datasets.

==> 2related-work.tex <==
\section{Related Work}

Over the past few years, researchers concentrate on intent identification across different domains. Flexible and adaptive intent class detection models have been developed for dynamic and evolving real-world applications. \cite{liao2023novel,kuzborskij2013n, scheirer2012toward, degirmenci2022efficient} focus on streaming data to identify evolving new classes using incremental learning. SENNE \citet{cai2019nearest}, IFSTC \cite{xia2021incremental}, SENC-MaS \cite{mu2017streaming}, SENCForest \cite{mu2017classification}, ECSMiner \citep{masud2010classification} aim at SENC problem (streaming emerging new class) on intents on streams. \newcite{sun2016online} work on emergence and disappearance of intents. 
\newcite{wang2020active} uses high dimensional data for streaming classification. \newcite{mullick2022framework} identifies multiple novel intents using a clustering framework. \cite{na2018dilof,zhan2021out,larson2019evaluation,yan2020unknown, zhou2022knn, firdaus2023multitask} detect new intents in the form of outlier detection. Unlike the previous single-intent detection models, which can easily utilize the utterance's sole intent to guide slot prediction, multi-intent SLU encounters the challenge of multiple intents, presenting a unique and worthwhile area of research.
AGIF~\cite{qin2020agif}, GL-GIN~\cite{qin2021gl}, \cite{gangadharaiah2019joint}, \cite{song2022enhancing} work on multiple intent identification problem but these approaches do not detect the sentence spans related to different intents. Based on Convert~\cite{henderson2019convert} backed framework, \cite{coope2020span} extract spans for different slots but does not extract and identify multiple intents.
